From Prisons to Programming: Fostering Self-Efficacy via Virtual Web Design Curricula in Prisons and Jails

Self-efficacy and digital literacy are key predictors to incarcerated people's success in the modern workplace. While digitization in correctional facilities is expanding, few templates exist for how to design computing curricula that foster self-efficacy and digital literacy in carceral environments. As a result, formerly incarcerated people face increasing social and professional exclusion post-release. We report on a 12-week college-accredited web design class, taught virtually and synchronously, across 5 correctional facilities across the United States. The program brought together men and women from gender-segregated facilities into one classroom to learn fundamentals in HTML, CSS and Javascript, and create websites addressing social issues of their choosing. We conducted surveys with participating students, using dichotomous and open-ended questions, and performed thematic and quantitative analyses of their responses that suggest students' increased self-efficacy. Our study discusses key design choices, needs, and recommendations for furthering computing curricula that foster self-efficacy and digital literacy in carceral settings.

==> qualitative.tex <==



% \section{Qualitative Analysis}

% \subsection{Self-Confidence and Perceived Benefits}

% \textbf{The class improved my self-confidence:}

% \begin{itemize}
%     \item \textit{"Yes it shows me that I can do it. It's never too late to learn something new."} - (p4)
%     \item \textit{"This class has given me more confidence in myself as well as using a computer."} - (p10)
%     \item \textit{"I never thought I could do anything like this."} - (p11)
%     \item \textit{"One of the best parts of this class were the 'aha!' moments where it's like 'I can code! I’m really doing it!'."} - (p15)
%     \item \textit{"Yes. At first, I was a shy person and now I’m not afraid to speak up. I’m better now about asking for help."} - (p16)
%     \item \textit{"It challenged me to stay focused and learn something new that I had zero background in."} - (p20)
%     \item \textit{"At first I didn't think I could do it, but now I know anything you put your mind to, you can really do it."} - (p21)
%     \item \textit{"Absolutely. As computer illiterate as I was, learning web design has sparked my thirst for attaining knowledge from this day forward."} - (p23)
%     \item \textit{"My self-confidence is on another level."} - (p27)
%     \item \textit{"Yes because it showed me how to do something that I felt was so hard."} - (p29)
%     \item \textit{"Yes because I feel confident about building a website and coding in HTML/CSS."} - (p31)
%     \item \textit{"This class has shown me that I am human again and I deserve to have a better quality of life post-incarceration."} - (p32)
% \end{itemize}

% \textbf{The class did not improve my self-confidence:}

% \begin{itemize}
%     \item \textit{"No because my confidence is in the almighty God, Jesus, my savior, teacher, and everything else."} - (p5)
%     \item \textit{"No, I just have low self-confidence anyway, but it was a great class and I enjoyed it."} - (p8)
%     \item \textit{"I mean... [name of other programming class] did most of that..."} - (p9)
%     \item \textit{"No"} - (p12)
% \end{itemize}

% \subsection{Perceived Best Parts of the Class}

% \textbf{Creating meaningful websites with newly acquired skills:}

% \begin{itemize}
%     \item \textit{"It was really awesome to see something that I built up from nothing but an idea and some characters turn out as well as this did. It was awesome to see something I made on the internet."} - (p9)
%     \item \textit{"The best part of the class was working on my own website and learning all the codes and how to use them. I have a whole new outlook on websites now."} - (p10)
%     \item \textit{"The opportunity to support victims of domestic violence through the creation of this website."} - (p13)
%     \item \textit{"For me the best part was learning a computer all over again after not using one in 21 years and then learning code at the same time."} - (p16)
% \end{itemize}

% \textbf{Inclusive and tailored instruction via breakout rooms:}

% \begin{itemize}
%     \item \textit{"Communication with TA's...individual instruction when needed."} - (p3)
%     \item \textit{"I think the best part of this class was the fact that there were no expectations put on us other than that we did our best. I also really appreciate the one-on-one time we were able to have with our TAs."} - (p7)
%     \item \textit{"The non-judgement completely inclusive atmosphere."} - (p11)
%     \item \textit{"A welcomed learning environment that let me escape for 4 hours a week. Learning the material."} - (p14)
%     \item \textit{"Working with people who took their time to explain how to code and made sure we understood."} - (p20)
%     \item \textit{"The instruction is the best part of the class. Our TA's are highly educated and dedicated, makes for a very stimulating course."} - (p26)
%     \item \textit{"The best part about this class was that I received all the help needed to be able to solve some obstacles I encountered throughout the class."} - (p29)
% \end{itemize}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% \subsection{Qualitative feedback}
% The post-course survey was completed by 33 students. When students were asked whether the class improved their self-confidence, and to explain their answer, 28 responded in the affirmative, 17 of which responded explicitly with "yes", 4 responded in the negative, and 1 did not respond to the question. Participants stated the following: 

% \textbf{The class improved my self-confidence:} "yes it show me that I can do it. It never to late to learn something new" - (p4). "This class has given me more confidence in myself as well as using a computer" - (p10). "I never thought I could do anything like this" - (p11). "One best parts of this class [were] the ‘aha!’ moment where it’s like ‘I can code! I’m really doing it!’. The self-possession, boost of confidence, and the satisfaction that I felt from participating in this class was an invaluable educational and relational experience in this collaborative learning environment" - (p15). "Yes. At first, I was a shy person and now I’m not afraid to speak up. I’m better now about asking for help" - (p16). "It challenged me to stay focused and learn something new that I had zero background in" - (p20). "At first I ain't think I could do, but now I know anything you put your mind to can you really do it" - (p21). "Absolutely. As computer illiterate as I was and learning web design has sparked my thirst for attaining knowledge this day forward. \martin{Also check my article I wrote for the course}" - (p23). "My self-confidence is on another level. \martin{Thanks to MIT Brave Behind Bars}" - (p27). "Yes because it showed me how to do something that I felt was so hard" - (p29). "Yes because I feel confident about building a website and coding in HTML/CSS" - (p31). "This class has shown me that I am human again and I deserve to have a better quality of life post-incarceration. Having access to so many bright young professionals has unlimited potential" - (p32).

% \textbf{The class did not improve my self-confidence:} "No because my confidence is in the almighty God JESUS MY savior teacher and everything else" - (p5). "No I just have low self-confidence any ways but it was a great class and I enjoyed it" - (p8). "I mean... \martin{[name of other programming class]} did most of that..." - (p9). "No" - (p12).


% When asked about what students perceived as the best part of the class, participants stated the following: 

% \textbf{Creating a meaningful websites with newly acquired skills:} "It was really awesome to see something that I built up from nothing but an idea and some characters turn as well as this did. It was awesome to see something I made on the internet" - (p9). "The best part of the class was working on my own website and learning all the codes and how to use them. I have a whole new out look on websites now" - (p10). "The opportunity to support victims of domestic violence through the creation of this website." - (p13). "For me the best part was learning a computer all over again after not using one in 21 years and then learning code at the same time so it was learning a new language but familiarizing myself with the keys, the commands and everything so it was amazing and extremely terrifying at the same time. I LOVED IT!" - (p16).

% \textbf{Inclusive and tailored instruction via breakout rooms:} "Communication with TA's...individual instruction when needed" - (p3). "I think the best part of this class was the fact that there were no Expectations put on us other than that we did our best. I also really appreciate the one-on-one time we were able to have with our TAs even if it was just to give feedback on our websites" - (p7). "The non-judgement completely inclusive atmosphere" - (p11). "A welcomed learning environment that let me escape for 4 hours a week. Learning the material." - (p14). "Working with people who took their time to explain how to code and made sure we understood" - (p20). "The instruction is the best part of the class. Our TA's are highly educated and dedicated, makes for a very stimulating course" - (p26). "The best part about this class was that I received all the help needed to be able to solve some obstacles I encountered throughout the class" - (p29).

